Robust Steady-State-Aware Model Predictive Control for Systems with Limited Computational Resources and External Disturbances

Model Predictive Control (MPC) is a powerful control strategy; however, its reliance on online optimization poses significant challenges for implementation on systems with limited computational resources. One possible approach to address this issue is to shorten the prediction horizon and adjust the conventional MPC formulation to enlarge the region of attraction. However, these methods typically introduce additional computational load. Recently, steady-state-aware MPC has been introduced to ensure output tracking and convergence to a given desired steady-state configuration while maintaining constraint satisfaction at all times without adding extra computational load. Despite its promising performance, steady-state-aware MPC does not account for external disturbances, which can significantly limit its applicability to real-world systems. This paper aims to advance the method further by enhancing its robustness against external disturbances. To achieve this, we adopt the tube-based design framework, which decouples nominal trajectory optimization from robust control synthesis, thereby requiring no additional online computational resources. Theoretical guarantees of the proposed methodology are shown analytically, and its effectiveness is assessed through simulations and experimental studies on a Parrot Bebop 2 drone.

==> extra.tex <==
%Explicit MPC~\cite{alessio2009survey, kvasnica2019complexity,  bemporad2021explicit} pre-computes and stores optimal control laws offline, significantly reducing online computational effort. Additionally, methods such as triggering mechanisms~\cite{sun2019robust, wang2020event} limit control updates to necessary instances, thereby alleviating computational load. Anytime MPC, which provides stability with minimal iterations, is another approach but does not guarantee constraint satisfaction~\cite{feller2018sparsity}. Another common approach to reduce computational complexity is to shorten the prediction horizon~\cite{sawma2018effect, pannek2011reducing}. As a result, the Region of Attraction (RoA) may be reduced, meaning the set of initial states for which the MPC problem remains feasible.


To enhance the robustness of MPC, modifications have been explored to traditional MPC frameworks. Robust MPC methods aim to ensure system performance under model uncertainties and external disturbances \cite{kothare1996robust}. These techniques include integrating robust optimization approaches and adjusting MPC structures to account for variations in system dynamics.

In this context, recent studies have investigated approaches to incorporate robustness directly into the MPC formulation. For instance, \cite{fathy2005dynamic} explores using a characterizing vector to account for steady-state configurations, thus ensuring robust output tracking and constraint satisfaction. Moreover, \cite{doan2015penalty} introduces a penalty term to address deviations from desired steady-state configurations, but challenges remain in determining the optimal configuration, particularly for piecewise constant references where sequences are not known in advance.

To overcome these limitations, our work proposes a steady-state-aware robust MPC that simultaneously addresses robustness and tracking of piecewise constant references. This approach ensures that the system converges to the desired steady-state configuration if feasible, or to the best admissible configuration while maintaining constraint satisfaction and robustness against disturbances. Our method improves upon previous strategies by providing a systematic way to handle both robustness and tracking without requiring prior knowledge of reference sequences.

